FT2Ra: A Fine-Tuning-Inspired Approach to Retrieval-Augmented Code Completion

The rise of code pre-trained models has significantly enhanced various coding tasks, such as code completion, and tools like GitHub Copilot. However, the substantial size of these models, especially large models, poses a significant challenge when it comes to fine-tuning them for specific downstream tasks. As an alternative approach, retrieval-based methods have emerged as a promising solution, augmenting model predictions without the need for fine-tuning. Despite their potential, a significant challenge is that the designs of these methods often rely on heuristics, leaving critical questions about what information should be stored or retrieved and how to interpolate such information for augmenting predictions. To tackle this challenge, we first perform a theoretical analysis of the fine-tuning process, highlighting the importance of delta logits as a catalyst for improving model predictions. Building on this insight, we develop a novel retrieval-based method, FT2Ra, which aims to mimic genuine fine-tuning. While FT2Ra adopts a retrieval-based mechanism, it uniquely adopts a paradigm with a learning rate and multi-epoch retrievals, which is similar to fine-tuning.In token-level completion, which represents a relatively easier task, FT2Ra achieves a 4.29% improvement in accuracy compared to the best baseline method on UniXcoder. In the more challenging line-level completion task, we observe a substantial more than twice increase in Exact Match (EM) performance, indicating the significant advantages of our theoretical analysis. Notably, even when operating without actual fine-tuning, FT2Ra exhibits competitive performance compared to the models with real fine-tuning.

==> sections/abstract.tex <==
% The advent of large language models (LLMs) has significantly enhanced a variety of coding tasks, such as code completion and tools like GitHub Copilot. However, the large size of these LLMs presents a considerable challenge when it comes to their fine-tuning for downstream tasks. As an alternative, retrieval-based methods have emerged as a promising solution, augmenting model predictions without the necessity for fine-tuning.
% Despite their potential, a significant challenge is that the designs of these methods are often heuristic, leaving unresolved questions regarding \textit{what information should be retrieved and how to interpolate this information into the predictions.}

% To address this challenge, we introduce a novel method, deeply rooted in a theoretical analysis of the fine-tuning process, which implies the significance of $\Delta logits$ as a catalyst for enhancing model predictions. Building on this insight, we developed the method \tool, which aims to emulate genuine fine-tuning. While \tool operates on a retrieval-based mechanism, it uniquely adopts a paradigm with a learning rate and multi-epoch iterations, which is similar to fine-tuning, .

% We evaluated \tool on both token-level and line-level completions. Our results demonstrate the effectiveness of \tool compared to state-of-the-art methods and the promising potential of \tool compared to genuine fine-tuning. For example, compared to the best of the baseline on pre-trained models, \tool achieves \fei{XX} accuracy boost on token-level completion and \fei{XX} EM increase on line-level completions. Remarkably, even in the absence of fine-tuning, \tool, when evaluated on pre-trained models, showcases competitive performance in line with models fine-tuned over \fei{XX} epochs.

% % Iterative Generation Through Memorization for Code Completion
% In recent times, code completion plugins like GitHub Copilot and Visual Studio IntelliCode have revolutionized the software development domain, substantially improving efficiency and reducing developers' cognitive loads. While these tools offer significant advantages, they primarily cater to generic code completion and often overlook domain-specific nuances, such as unique API calls or intricate project-specific variable naming conventions. This limitation becomes even more evident at the repository level, where interdependencies within files aren't considered by general-purpose models.

% The direct approach to address these domain-specific gaps is to fine-tune the large language models with project data. However, due to their sheer size and complexity, frequent fine-tuning becomes impractical and costly. To overcome this, retrieval-augmented language models (R-LMs) have been introduced. While these models bring advantages, they are not without flaws. For instance, many R-LMs lack theoretical foundation and depend solely on empirical results for validation. Methods like KNN-LM, though innovative, do not effectively harness the model's latent information, often treating correct and erroneous predictions uniformly.

% In this study, we introduce an innovative approach to tackle the above challenges: an iterative generation method via KNN for code completion. Our method, grounded in theoretical principles, offers more than just a probability interpolation—it delivers iterative outcomes reminiscent of the fine-tuning process. It holds the dual advantage of being effective both on models that haven't been fine-tuned and those that have undergone the process. Furthermore, our proposed method excels in deriving insights from erroneous predictions, showing exceptional promise, especially in scenarios with limited datasets.
